TurboFNO: High-Performance Fourier Neural Operator with Fused FFT-GEMM-iFFT on GPU

Fourier Neural Operators (FNO) are widely used for learning partial differential equation solution operators. However, FNO lacks architecture-aware optimizations,with its Fourier layers executing FFT, filtering, GEMM, zero padding, and iFFT as separate stages, incurring multiple kernel launches and significant global memory traffic. We propose TurboFNO, the first fully fused FFT-GEMM-iFFT GPU kernel with built-in FFT optimizations. We first develop FFT and GEMM kernels from scratch, achieving performance comparable to or faster than the closed-source SOTA cuBLAS and cuFFT. Additionally, our FFT kernel integrates a built-in high-frequency truncation, input zero-padding, and pruning feature to avoid additional memory copy kernels. To fuse the FFT and GEMM workloads, we propose an FFT variant in which a single thread block iterates over the hidden dimension, aligning with the $k$-loop in GEMM. Additionally, we design two shared memory swizzling patterns to achieve 100\% memory bank utilization when forwarding FFT output to GEMM and enabling the iFFT to retrieve GEMM results directly from shared memory.Experimental result on an NVIDIA A100 GPU shows TurboFNO outperforms PyTorch, cuBLAS, and cuFFT by up to 150\%.

==> setting/author_ieee.tex <==
%%% plain version
\newcommand{\EqContribMark}{$^{\bullet}$}
\newcommand{\UcrMark}{\IEEEauthorrefmark{1}}
\newcommand{\IuMark}{\IEEEauthorrefmark{2}}
\newcommand{\AnlMark}{\IEEEauthorrefmark{3}}
\newcommand{\FsuMark}{\IEEEauthorrefmark{4}}
\newcommand{\UiowaMark}{\IEEEauthorrefmark{5}}
\newcommand{\CasMark}{\IEEEauthorrefmark{6}}
\newcommand{\UhustonMark}{\IEEEauthorrefmark{7}}

\newcommand{\CorrespondingAuthorMark}{$^{\star}$}

%%% revised version
\renewcommand{\EqContribMark}{$^{\bullet}$}
\renewcommand{\UcrMark}{$^\triangleright$}
\renewcommand{\IuMark}{$^\circ$}
\renewcommand{\AnlMark}{$^\diamond$}
\renewcommand{\FsuMark}{$^\P$}
\renewcommand{\UiowaMark}{$^\S$}
\renewcommand{\CasMark}{$^\|$}
\renewcommand{\UhustonMark}{$^\times$}

\author
{\normalsize\null\\[-4.2ex] %% jtian: this works to shrink the title-authorblock spacing anyway.
\begin{minipage}{\linewidth}\centering
Jinyang Liu\,\UhustonMark\EqContribMark,
Jiannan Tian\,\IuMark\EqContribMark,
Shixun Wu\,\UcrMark\EqContribMark,%
    \thanks{\hspace{-1em}\EqContribMark\,Jinyang Liu, Jiannan Tian, and Shixun Wu contributed equally to this work.}
Sheng Di\,\AnlMark\CorrespondingAuthorMark,
Boyuan Zhang\,\IuMark,
Robert Underwood\,\AnlMark,
Yafan Huang\,\UiowaMark,\\
Jiajun Huang\,\UcrMark,
Kai Zhao\,\FsuMark,
Guanpeng Li\,\UiowaMark,
Dingwen Tao\,\CasMark\CorrespondingAuthorMark, 
    \thanks{\hspace{-1em}\CorrespondingAuthorMark\,Corresponding authors: Sheng Di, Dingwen Tao.}
Zizhong Chen\,\UcrMark,
Franck Cappello\,\AnlMark
\\[.9ex]
% \normalsize
% \IEEEauthorrefmark{1} 
\UhustonMark\,%
University of Houston, Houston, TX, USA;\ \ \texttt{jliu217@central.uh.edu}\\
\IuMark\,%
Indiana University, Bloomington, IN, USA;\ \ \texttt{\,\string{\,jti1,\,bozhan\,\string}@iu.edu}\\
\UcrMark\,%
University of California, Riverside, CA, USA;\ \ \texttt{\string{\,swu264,\,jhuan380\,\string}@ucr.edu, chen@cs.ucr.edu}\\
% \IEEEauthorrefmark{2}
% \IEEEauthorrefmark{3}
\AnlMark\,%
Argonne National Laboratory, Lemont, IL, USA;\ \ \texttt{\string{\,sdi1,\,runderwood\,\string}@anl.gov, cappello@mcs.anl.gov}\\
% \IEEEauthorrefmark{4}
\UiowaMark\,%
University of Iowa, Iowa City, IA, USA;\ \ \texttt{\string{\,yafan-huang,\,guanpeng-li\,\string}@uiowa.edu}\\
% \IEEEauthorrefmark{5}
\FsuMark\,%
Florida State University, Tallahassee, FL, USA;\ \ \texttt{kai.zhao@fsu.edu}\\
\CasMark\,%
SKLP, Institute of Computing Technology, Chinese Academy of Sciences, China;\ \ \texttt{taodingwen@ict.ac.cn}
%% jtian: \\[-3.0ex] just works to reduce the author block spacing and I don't know how.
\end{minipage}\\[-3ex]
}


==> setting/grand-preamble.tex <==
%%%%%% graphics
\usepackage{hyperref}
\usepackage{graphicx}
\usepackage{xcolor}
\definecolor{B}    {HTML}{2b66d3}   %% blue, light
\definecolor{B2}   {HTML}{003399}   %% blue, dark 
\definecolor{Bv}   {HTML}{0000EB}   %% blue, vibrant
\definecolor{R}    {HTML}{c9171e}
\definecolor{R2}   {HTML}{d7003a}
\definecolor{INK}  {HTML}{595857}
\definecolor{Y}    {HTML}{f1c40f}
\definecolor{G}    {HTML}{009a00}
\definecolor{GRAY} {HTML}{808080}
\definecolor{MAUVE}{HTML}{9400D1}


%%%%%%%%%%% defined symbols, terminology
%% \scshape only when camera-ready
\newcommand{\cusz}{{\scshape cuSZ}}
%% mbox to hyphenate without being breakable
\newcommand{\cuszinterp}{\mbox{\textsc{cuSZ}-$i$}}
\newcommand{\thiswork}{\cuszinterp}
\newcommand{\ginterp}{\mbox{\textit{G-Interp}}}
\newcommand{\ginterpalter}{\ginterp}
\newcommand{\bitcomp}{Bitcomp-lossless}
\newcommand{\datasetname}[1]{{\ttfamily #1}}
\newcommand{\datafieldname}[1]{{\ttfamily #1}}


%%%%% tabular
\usepackage{array}      %% https://tex.stackexchange.com/q/338009
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{tabu}       %% friendly when coloring

% \usepackage{flushend}
\usepackage[T1]{fontenc}

\input{setting/module_text_func}	%% todo must use after `module_color'
\input{setting/module_text_macros}
\input{setting/module_tikz}

\usepackage{anyfontsize}

%%%% math
\usepackage{amsmath}    %% \text in mathmode
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}    %% may cause conflict
% \usepackage{mathabx}
\usepackage{mathtools}
\usepackage{bm}
\newtheorem{theorem}{Theorem}


%%%%
\usepackage{caption}
\usepackage{subcaption}
\captionsetup[figure]{font=small, labelfont=small}
\captionsetup[table]{font=small, labelfont=small}
% \captionsetup[algorithm]{font=small, labelfont=small}
\setlength{\textfloatsep}{6pt}
\setlength\abovecaptionskip{3pt}
\setlength{\abovedisplayskip}{2pt}
\setlength{\belowdisplayskip}{2pt}
\setlength{\abovedisplayshortskip}{2pt}
\setlength{\belowdisplayshortskip}{2pt}

% \captionsetup[algorithm]{font=small}%, singlelinecheck=off}
% \captionsetup[figure]{font=small, skip=1ex}
% \captionsetup[table]{font=small, skip=1ex}
\captionsetup[subfigure]{font=small, labelfont=small}
% \captionsetup[subtable]{font=small, labelfont=small}
% \captionsetup{width=.8\linewidth, justification = raggedright}
% \captionsetup{width=.8\linewidth, justification = centering}


\newcommand{\WeModifyIeeeTemplateToEnablePageNumber}{
	\thispagestyle{plain}\pagestyle{plain}}

%%%%%% enhanced text
% \usepackage{lipsum}%% generate testing text
\usepackage[normalem]{ulem}
% \usepackage{todonotes}
\usepackage{stackengine}
\usepackage{rotating}	%% dependency of turn


%% jtian: comment/circumvent the following for texpad convenience 
%\usepackage[inkscapeformat=png]{svg}


%% last step, change font conveniently
\usepackage[scale=.92]{tgheros}

\renewcommand*{\ttdefault}{lmtt}

\hypersetup{
	pdftitle={cuSZ-i: High-Ratio Scientific Lossy Compression on GPUs with Optimized Multi-Level Interpolation},
	pdfauthor={Liu, Tian, Wu ,et al.},
	pdfsubject={cuSZ-i, camera-ready (in progress)},
	pdfkeywords={GPU; compression; data quality; lossy; error bound; HPC; scientific data}
}


%% https://tex.stackexchange.com/a/29146
%% SCtable, SCfigure
\usepackage[outercaption]{sidecap}
\sidecaptionvpos{figure}{b}
\sidecaptionvpos{table}{b}

==> setting/module_text_func.tex <==
\usepackage{url, hyperref}                  %% hyperlink
\hypersetup{
    colorlinks, linkcolor=RoyalBlue, citecolor=RoyalBlue, urlcolor=RoyalBlue,
    allcolors=RoyalBlue,
    breaklinks=true,
    pdfborder={0 0 0}}

\usepackage{enumitem}                       %% enhanced items
\usepackage{lipsum}                         %% pseudo texts
%%% fully working and highly tuned, but I disable the whole algo functionality anyway
% \usepackage[plain]{algorithm}       		% algo%rithm
% \floatstyle{plaintop}
% \usepackage{algpseudocode}
% \algrenewcommand{\alglinenumber}[1]{{\scriptsize\bfseries\ttfamily\color{R}#1}}
% \floatstyle{plaintop}
% \restylefloat{algorithm}

% \usepackage{xurl}       %%% try breaking long URLs
% \usepackage{breakurl}


% \usepackage{xpatch}% specifically for fixing indentation, thanks to https://tex.stackexchange.com/questions/294840/indent-algorithmic-outside-of-a-block
% \makeatletter
% \xpatchcmd{\algorithmic}{\ALG@tlm\z@}{\ALG@tlm\z@\leftmargin 10pt}{}{}
% \makeatother


\usepackage{listings}						%% code listing
\lstset{
    basicstyle=\ttfamily\small,     %%% string settings
    stringstyle=\color{R},
    keywordstyle=\color{B2}\bfseries,
    commentstyle=\color{gray},
    tabsize=2,
    breaklines=true,
    showstringspaces=false,
    showspaces=false,
    %backgroundcolor=\color{gray!4}, 
    xleftmargin=6pt,
    framexleftmargin=6pt,
    framesep=0pt,
    numberstyle=\bfseries\ttfamily\scriptsize\color{R},
    numbers=left, % {none, left, right}; position of line number
    numbersep=6pt, % how far the line-numbers are from the code
    stepnumber=1, % the step between two line-numbers. If it's 1, each line will be numbered
    escapeinside={Ω}{≈}
}

\usepackage{setspace}                       % spacing

\usepackage{soul}%% \hl{} and \st{}


==> setting/module_text_macros.tex <==
\ifx\UseACMTemplate\undefined
\else
    %% ACM
    \newcommand{\SEC}{\textcolor{black}{\S\hbox{\kern 0.1667em}}}
    \newcommand{\FIG}{\textcolor{black}{Figure~}}
    \newcommand{\TAB}{\textcolor{black}{Table~}}
\fi

\ifx\UseIEEETemplate\undefined
\else
    %% IEEE
    \newcommand{\SEC}{\textcolor{black}{\S\hbox{\kern 0.1667em}}}
    \newcommand{\FIG}{\textcolor{black}{Fig.\hbox{\kern 0.1667em}}}
    \newcommand{\TAB}{\textcolor{black}{TABLE~}}
\fi


\newcommand{\warichu}[3]{\footnotesize\begin{tabular}{@{}#3@{}}#1\\#2\end{tabular}}


\newcommand{\TABLETITLE}{\BOLD\color{Bv}}
\newcommand{\TABLECAPTION}{\color{gray}\scriptsize}

\newcommand{\YES}{$\bullet$}
\newcommand{\semiYES}{$\circ$}

%% table formatting

\newcommand{\lorenzond}[1]{\prescript{#1}{I}\ell} %% https://tex.stackexchange.com/a/11566
\newcommand\hfilll{\hspace{0pt plus 1filll}} %% https://tex.stackexchange.com/a/271872

%% ////////////////////////////////////////////////////////////////
%% hyphenation
\hyphenation{quan-ti-za-tion}
\hyphenation{chunk-wise}
\hyphenation{pre-dic-tion-quan-ti-za-tion}
\hyphenation{post-analysis}

\newcommand{\quantcode}{quant-code}


\newcommand{\CONSTEXPR}{{\color{HLCOLOR}constexpr}}
\newcommand{\VOLATILE}{{\color{HLCOLOR}volatile}}
\newcommand{\REFERENCE}{{\color{HLCOLOR}reference}}
\newcommand{\CAPTURE}{{\color{HLCOLOR}capture}}
\newcommand{\INLINEIF}{{\textbf{if}}}

\newcommand{\AlgoMark}[2][Y!40]{\hspace*{-\fboxsep}\colorbox{#1}{#2}}


\colorlet{HLCOLOR}{B}
\colorlet{TableAltColor}{gray!20}


\newcommand{\FloatBodyStyle}{\centering\small\fontfamily{lmr}\selectfont}
\newcommand{\NoBcBestCr}[1]{\color{RoyalBlue} \usefont{OT1}{cmr}{bx}{n} {#1}}
\newcommand{\BestCr}[1]{\color{RoyalBlue} \usefont{OT1}{cmr}{bx}{n} {#1}}
\newcommand{\SecondbestCr}[1]{\color{black} \underline{#1}}

==> setting/module_tikz.tex <==
\usepackage{tikz}
\usetikzlibrary{positioning}        %% must-have
\usetikzlibrary{shapes.multipart}   %% multiline node, should use as default
\usetikzlibrary{shapes.geometric}   %% diamond etc
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}        %% e.g., {[left]Bar}-{[right]Bar}
% \usetikzlibrary{decorations.text}
% \usetikzlibrary{decorations.pathreplacing}
% \usepgflibrary{decorations.markings}
\usetikzlibrary{backgrounds}
\usetikzlibrary{patterns}
\usetikzlibrary{fit}


\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{groupplots}

\newcommand*\Circled[1]{% require `tikz`
	\tikz[baseline=(char.base)]{%
		\node[shape=circle, draw=none, fill=gray!40, thick, inner sep=0.6pt] (char) {%
			\textcolor{black}{\sffamily#1}}; }}
